Design Assurance Evaluation of Microcontrollers for safety critical Avionics

Dealing with Commercial off-the-shelf (COTS) com- ponents is a daily business for avionic system manufacturers. They are necessary ingredients for hardware designs, but are not built in accordance with the avionics consensus standard DO- 254 for Airborne Electronic Hardware (AEH) design. Especially for complex COTS hardware components used in safety critical AEH, like Microcontroller Units (MCUs), additional assurance activities have to be performed. All of them together shall form a convincing confident, that the hardware is safe in its intended operation environment. The focus of DO-254 is one approach called Design Assurance (DA). Its aim is to reduce design errors by adherence of prescribed process objectives for the entire design life cycle. The effort for certain COTS assurance activities could be reduced if it is possible to demonstrate, that the COTS design process is based on similar effective design process guide- lines to minimize desgin errors. In the last years, semiconductor manufacturers released safety MCUs in compliance to the ISO 26262 standard, dedicated for the development of functional safe automotive systems. These products are COTS components in the sense of avionics, but they are also developed according to a process that focuses on reduction of design errors. In this paper an evaluation is performed to figure out if the ISO 26262 prescribes a similar DA approach as the DO-254, in order to reduce the COTS assurance effort for coming avionic systems.

==> relatedWork.tex <==


%AVSI AFE 43 and the modeling of microprocessors that they started with but somewhat failed with.

%For the most \ac{cots} components no comparable approach is practised~\cite{FAA.2001}. This is explainable since \ac{cots} components are targeted to domains with different claims according to design and safety goals. 

%Acc. to crossdomain Paper: Nur die DAL und mit einander zu vergleichen geht nicht. Sie haben einfach zu unterschiedliche Zwecke und Ursprünge. Eine echte Cross-Domain Äquvivalence wird wohl nicht erreichbar sein. (Achtung, das ist garnicht mein Ziel)


